Augmenting Document Representations for Dense Retrieval with Interpolation and Perturbation

Dense retrieval models, which aim at retrieving the most relevant document for an input query on a dense representation space, have gained considerable attention for their remarkable success. Yet, dense models require a vast amount of labeled training data for notable performance, whereas it is often challenging to acquire query-document pairs annotated by humans. To tackle this problem, we propose a simple but effective Document Augmentation for dense Retrieval (DAR) framework, which augments the representations of documents with their interpolation and perturbation. We validate the performance of DAR on retrieval tasks with two benchmark datasets, showing that the proposed DAR significantly outperforms relevant baselines on the dense retrieval of both the labeled and unlabeled documents.

==> 0ablation_table.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table}
\centering
\begin{center}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}[t]{l|cccccc}
%\Xhline{2\arrayrulewidth}
\toprule
%\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multicolumn{1}{c|}{} &\textbf{MRR} &\textbf{MAP} &\textbf{R@20} &\textbf{R@5}\\
%\hline
\midrule
\multirow{1}{*}{DAR (Ours)}
 & \textbf{42.92} & \textbf{27.12} & \textbf{75.04} & \textbf{57.62}\\
\multirow{1}{*}{w/o Perturbation}
 & 41.26 & 26.19 & 73.68 & 55.37\\
\multirow{1}{*}{w/o Interpolation}
 & 40.40 & 25.70 & 73.41 & 55.29\\
\midrule
\multirow{1}{*}{DPR}
 & 39.55 & 25.61 & 72.94 & 54.02\\
\bottomrule
%\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{center}
\vspace{-0.15in}
\caption{\small Ablation studies of DAR on the NQ dataset.}
\label{tab:ablation}
\vspace{-0.15in}
\end{table}

==> 0batch_fig.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.43\textwidth]{batch_line.pdf}
\end{center}
\vspace{-0.2in}
\caption{\small R@20 on the NQ with varying batch sizes.
}
\vspace{-0.05in}
\label{fig:batch_line}

\end{figure}

==> 0copy.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table*}
\centering
\begin{center}
\resizebox{\width}{!}{
\begin{tabular}[t]{ll|ccccccc}
\toprule
%\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multicolumn{2}{c|}{} & \textbf{MRR} & \textbf{MAP} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1} \\
%\hline
\midrule
\multirow{4}{*}{NQ} 
& BM25 & - & - & 73.7 & 59.1 & - & - & - \\
& DPR & 39.55 & 25.61 & 83.77 & 72.94 & 64.79 & 54.02 & 27.45 \\
& DGEN & 40.00 & 24.93 & 83.46 & 72.13 & 65.04 & 55.46 & 27.67 \\
& DAR & \textbf{42.92} & \textbf{27.12} & \textbf{84.18} & \textbf{75.04} & \textbf{67.78} & \textbf{57.62} & \textbf{30.42} \\
\hline
\multirow{4}{*}{TQA} 
& BM25 & - & - & 76.7 & 66.9 & - & - & - \\
& DPR & 44.29 & 27.24 & 80.50 & 71.07 & 65.06 & 57.74 & 33.63  \\
& DGEN &  &  &  &  &  &  &  \\
& DAR & \textbf{46.73} & \textbf{28.21} & \textbf{81.44} & \textbf{72.47} & \textbf{66.28} & \textbf{59.12} & \textbf{36.55} \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.15in}
\caption{Retrieval results on the NQ and TQA datasets. For BM25, we report the results from~\cite{karpukhin2020dpr}. The best performance is marked in \textbf{bold}.}
\label{tab:main}
\vspace{-0.15in}
\end{table*}

==> 0efficiency_time_memory.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table}
\centering
\begin{center}
\resizebox{0.4\textwidth}{!}{
\renewcommand{\arraystretch}{0.9}
\begin{tabular}[h]{l|ccc}
%\Xhline{2\arrayrulewidth}
\toprule
%\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multicolumn{1}{c|}{} &\textbf{Memory (MiB)} &\textbf{Time (Min.)} &\textbf{Relative Time} \\
%\hline
\midrule
\multirow{1}{*}{DPR}
 & 22,071 & 19 & 1.00\\
\multirow{1}{*}{DPR w/ QA}
 & 22,071 & 41 & 2.16\\
 \multirow{1}{*}{DPR w/ DA}
 & 22,071 & 38 & 2.00\\
 \multirow{1}{*}{DPR w/ AR}
 & 38,986 & 29 & 1.53 \\
\multirow{1}{*}{DAR (Ours)}
 & 22,071 & 21 & 1.11\\
\bottomrule
%\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{center}
\vspace{-0.175in}
\caption{\small Maximum memory usage and time for training a DPR model per epoch.}
\label{tab:efficiency_tiem_memory}
\vspace{-0.2in}
\end{table}

==> 0qar_table.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table}[ht]
        \vspace{-0.175in}
        \centering
        \begin{center}
        \resizebox{0.48\textwidth}{!}{
        %\renewcommand{\arraystretch}{0.95}
        \begin{tabular}[t]{l|ccccccc}
        \toprule
        \multicolumn{1}{c|}{} & \multicolumn{3}{c}{\textbf{Natural Questions (NQ)}} & \multicolumn{3}{c}{\textbf{TriviaQA (TQA)}} \\
        \cmidrule(l{2pt}r{2pt}){2-4} \cmidrule(l{2pt}r{2pt}){5-7} 
         & \textbf{T-100} & \textbf{T-20} & \textbf{T-5} & \textbf{T-100} & \textbf{T-20} & \textbf{T-5} \\
        %\multicolumn{1}{c|}{} & \textbf{MRR} & \textbf{MAP} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1}\\
        %\hline
        \midrule
        \multirow{1}{*}{BM25} & 78.25 & 62.94 & 43.77 & 83.15 & 76.41 & 66.28 \\
        \midrule
        \multirow{1}{*}{DPR} & 83.77 & 72.94 & 54.02 & 80.50 & 71.07 & 57.74 \\
        \multirow{1}{*}{DPR w/ QA} & 83.46 & 72.13 & 55.46 & 80.76 & 71.88 & 59.14\\
        \multirow{1}{*}{DPR w/ DA} & 83.68 & 72.83 & 55.51 & 80.42 & 71.55 & 58.64\\
        \multirow{1}{*}{DPR w/ AR} & 83.60 & 73.41 & 55.51 & 80.65 & 71.68 & 58.09\\
        \midrule
        \multirow{1}{*}{DAR (Ours)} & \textbf{84.18 }& \textbf{75.04} & \textbf{57.62} & \textbf{81.30} & \textbf{72.66} & \textbf{59.88} \\
        \multirow{1}{*}{QAR (Ours)} & \textbf{84.21} & \textbf{74.76} & \textbf{57.51} & \textbf{80.91} & \textbf{72.12} & \textbf{59.94} \\
        \bottomrule
        \end{tabular}
        }
        \end{center}
        \vspace{-0.15in}
        \captionof{table}{\small Retrieval results on NQ and TQA datasets, including the variant of our model -- QAR: applying data augmentation techniques to queries instead of documents. The best model and the second best model among dense retrievers are denoted in bold, which we aim to improve in this work.}
        \label{tab:qar}
    \vskip -0.05in
\end{table}



% \begin{table*}
% \centering
% \begin{center}
% \resizebox{1.0\textwidth}{!}{
% \begin{tabular}[t]{l|ccccccccccccccc}
% \toprule
% \multicolumn{1}{c|}{} & \multicolumn{7}{c}{\textbf{NQ}} & \multicolumn{7}{c}{\textbf{TQA}} \\
% \cmidrule(l{2pt}r{2pt}){2-8} \cmidrule(l{2pt}r{2pt}){9-15} 
%  & \textbf{MRR} & \textbf{MAP} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1} & \textbf{MRR} & \textbf{MAP} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1} \\
% %\multicolumn{1}{c|}{} & \textbf{MRR} & \textbf{MAP} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1}\\
% %\hline
% \midrule
% \multirow{1}{*}{BM25}
%  & 32.46 & 20.78 & 78.25 & 62.94 & 54.46 & 43.77 & 22.11 & 55.28 & 34.85 & 83.15 & 76.41 & 71.74 & 66.28 & 46.30 \\
% \midrule
% \multirow{1}{*}{DPR}
%  &39.55 & 25.61 & 83.77 & 72.94 & 64.79 & 54.02 & 27.45 & 44.29 & 27.24 & 80.50 & 71.07 & 65.06 & 57.74 & 33.63\\
% \multirow{1}{*}{DPR w/ QA}
%  & 40.00 & 24.93 & 83.46 & 72.13 & 65.04 & 55.46 & 27.67 & 46.27 & 28.08 & 80.76 & 71.88 & 66.24 & 59.14 & 35.90 \\
% \multirow{1}{*}{DPR w/ DA} & 41.28 & 26.60 & 83.68 & 72.83 & 65.24 & 55.51 & 29.31 & 46.08 & 27.82 & 80.42 & 71.55 & 65.92 & 58.64 & 35.85\\
% \multirow{1}{*}{DPR w/ AR} & 41.18 & 26.04 & 83.60 & 73.41 & 66.34 & 55.51 & 29.11 & 45.13 & 27.57 & 80.65 & 71.68 & 65.72 & 58.09 & 34.52\\
% \multirow{1}{*}{DAR (Ours)}
%  & \textbf{42.92} & \textbf{27.12} & \textbf{84.18} & \textbf{75.04} & \textbf{67.78} & \textbf{57.62} & \textbf{30.42} & \textbf{47.32} & \textbf{28.70} & \textbf{81.30} & \textbf{72.66} & \textbf{67.24} & \textbf{59.88} & \textbf{36.94}\\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-0.175in}
% \caption{\small Retrieval results on NQ and TQA datasets. BM25 is the sparse retrieval model, whereas others are dense retrieval models. The numbers in bold denote the best model among dense retrieval models, which we aim to improve in this work.}
% \label{tab:main}
% \vspace{-0.15in}
% \end{table*}

==> 0reader_fig.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.43\textwidth]{reader.pdf}
\end{center}
\vspace{-0.15in}
\caption{\small Exact Match (EM) scores for a reader on the NQ with a varying number of retrieved documents.
}
\vspace{-0.2in}
\label{fig:reader}

\end{figure}

==> 0seenunseen_table.tex <==
\aboverulesep=0ex
\belowrulesep=0ex

\begin{table}
\centering
\vspace{-0.05in}
\begin{center}
\resizebox{0.475\textwidth}{!}{
\begin{tabular}[t]{ll|ccccc}
%\Xhline{2\arrayrulewidth}
\toprule
%\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multicolumn{2}{c|}{} & \textbf{R@100} & \textbf{R@20} & \textbf{R@10} & \textbf{R@5} & \textbf{R@1}\\
%\hline
\midrule
\multirow{2}{*}{Labeled}
& DPR & 38.86 & 28.48 & 23.10 & 17.20 & 6.51 \\
& DAR (Ours) & \textbf{40.39} & \textbf{30.44} & \textbf{24.68} & \textbf{19.09} & \textbf{7.34} \\
\hline
\multirow{2}{*}{Unlabeled}
& DPR & 79.78 & 67.15 & 58.20 & 46.95 & 20.94\\
& DAR (Ours) & \textbf{80.53} & \textbf{69.78} & \textbf{61.66} & \textbf{50.69} & \textbf{23.07}\\
\bottomrule
%\Xhline{2\arrayrulewidth}
\end{tabular}
}
\end{center}
\vspace{-0.15in}
\caption{\small Retrieval results on the labeled and unlabeled samples in the NQ dataset.
%Accuracy (Acc@K) measures the proportion of correctly retrieved seen/unseen documents among K seen/unseen candidate documents. The best performance is marked in \textbf{bold}.
}
\label{tab:seenunseen}
\vspace{-0.2in}
\end{table}
